Multi-Agent Path Finding via Tree LSTM

In recent years, Multi-Agent Path Finding (MAPF) has attracted attention from the fields of both Operations Research (OR) and Reinforcement Learning (RL). However, in the 2021 Flatland3 Challenge, a competition on MAPF, the best RL method scored only 27.9, far less than the best OR method. This paper proposes a new RL solution to Flatland3 Challenge, which scores 125.3, several times higher than the best RL solution before. We creatively apply a novel network architecture, TreeLSTM, to MAPF in our solution. Together with several other RL techniques, including reward shaping, multiple-phase training, and centralized control, our solution is comparable to the top 2-3 OR methods.

==> table/computational_resource.tex <==
\begin{table}[t]
    \centering
    
    \begin{tabular}{lccc}
        \toprule
        Experiment & \#GPU & Batch Size & \#CPU cores \\
        \midrule
        Phase-1 & 4 & 2048 & 960 \\
        Phase-2 & 4 & 1536 & 880 \\
        Phase-3-50 & 4 & 1536 & 880 \\
        Phase-3-80 & 4 & 1024 & 880 \\
        Phase-3-100 & 4 & 1024 & 880 \\
        Phase-3-200 & 6 & 512 & 1440 \\
        \bottomrule
    \end{tabular}
    
    \caption{Computational resources of the experiments.}
    \label{tab:computational_resource}
\end{table}

==> table/main-result-old.tex <==
\begin{table*}[t]
    \centering
    \begin{tabular}{llrcrlrr}
        \toprule
        Test Stage & Model & \#agents & Map Size & \#cities & Arrival\% & Env. Reward & Avg. Time/s \\
        \midrule
        \tt{Test\_00} & Phase-III-50 & 7 & $30 \times 30$ & 2 & $91.4 \pm 10.0$ & $.942 \pm .055$ & 7.420 \\
        \tt{Test\_01} & Phase-III-50 & 10 & $30 \times 30$ & 2 & $91.0 \pm 9.9$ & $.942 \pm .056$ & 8.650 \\
        \tt{Test\_02} & Phase-III-50 & 20 & $30 \times 30$ & 3 & $84.0 \pm 21.1$ & $.914 \pm .092$ & 17.064 \\
        \tt{Test\_03} & Phase-III-50 & 50 & $30 \times 35$ & 3 & $84.4 \pm 14.3$ & $.908 \pm .071$ & 33.392 \\
        \tt{Test\_04} & Phase-III-80 & 80 & $35 \times 30$ & 5 & $62.0 \pm 13.4$ & $.815 \pm .037$ & 46.940 \\
        \tt{Test\_05} & Phase-III-80 & 80 & $45 \times 35$ & 7 & $63.1 \pm 13.8$ & $.814 \pm .057$ & 65.053 \\
        \tt{Test\_06} & Phase-III-80 & 80 & $40 \times 60$ & 9 & $65.3 \pm 14.7$ & $.825 \pm .060$ & \\
        \tt{Test\_07} & Phase-III-80 & 80 & $60 \times 40$ & 13 & $70.6 \pm 10.6$ & $.850 \pm .042$ & \\
        \tt{Test\_08} & Phase-III-80 & 80 & $60 \times 60$ & 17 & $75.6 \pm 7.6$ & $.867 \pm .032$ & \\
        \tt{Test\_09} & Phase-III-100 & 100 & $80 \times 120$ & 21 & $53.1 \pm 15.3$ & $.783 \pm .060$ & \\
        \tt{Test\_10} & Phase-III-100 & 100 & $100 \times 80$ & 25 & $65.4 \pm 12.2$ & $.823 \pm .049$ & \\
        \tt{Test\_11} & Phase-III-200 & 200 & $100 \times 100$ & 29 & $54.0 \pm 7.5$ & $.746 \pm .037$ & 564.030 \\
        \tt{Test\_12} & Phase-III-200 & 200 & $150 \times 150$ & 33 & $57.1 \pm 5.3$ & $.762 \pm .021$ & 1545.162 \\
        \tt{Test\_13} & Phase-III-200 & 400 & $150 \times 150$ & 37 & $32.1 \pm 5.1$ & $.684 \pm .017$ & 2402.670 \\
        \tt{Test\_14} & Phase-III-200 & 425 & $158 \times 158$ & 41 & & & \\
        \bottomrule
    \end{tabular}
    \caption{Performance of our models in 15 test stages. (old)}
    \label{tab:main-result-old}
\end{table*}

